Solving degenerate 2D frustration-free spin systems in sub-exponential time

We give an improved analysis of approximate ground space projectors (AGSPs) to obtain a sharp error reduction bound in the setting a degenerate ground space. The improved tools imply that the recently proven 2D area law directly extends to sub-exponentially degenerate ground spaces and also yields a sub-exponential-time classical algorithm to compute the ground states. This time complexity cannot be improved beyond sub-exponential, even for the special case of classical unfrustrated systems in 2D.

==> MPO.tex <==
\begin{tikzpicture}[scale=1/22, every node/.style={scale=0.9}]
\newcommand\m{5}
\newcommand\s{8}
\node[right] at (-13,9){$\iAGSP$};
\node[right] at (-13,-20){$\mathbb T$};
	\foreach\j in{1,3,...,77}{%2*(\s*\m-1)-1}
		\foreach\l in{-1,5,11,17}
	\draw(6*\j/2,\l)--(6*\j/2+4,\l);
}

	\foreach\i in {0,1,...,7}{
		\foreach\l in{2,8,14,20}
    \draw ({6*\m*(\i+1)-2},\l+1)rectangle(6*\m*\i,\l-1);
	\foreach\j in{0,1,...,4}{
		\foreach\l in{2,8,14,20}
        \draw[decorate,decoration={snake,segment length=1mm,amplitude=.1mm}](6*\m*\i+6*\j,\l)--(6*\m*\i+6*\j+4,\l);
        }
    }
    \draw[thick]({3*\m-1},-20)--({6*\m*(\s-0.5)-1},-20);
	\foreach\i in {0,1,...,7}{%\s-1}{
    \draw[thick] ({6*\m*(\i+0.5)-1},-10)--({6*\m*(\i+0.5)-1},-30);
    \fill({6*\m*(\i+0.5)-1},-20)circle(2);
}
\end{tikzpicture}


==> MPS2.tex <==
% !TeX root = main.tex

\begin{tikzpicture}[scale=.5, every node/.style={scale=0.9}]

	\draw[very thick](-10,.5)--(9,.5);

	\draw[color=gray](-11,-1.1)--(8.8,-1.1)--(8/1.1,1/1.1)--(-10/1.1,1/1.1); 
\draw[decorate,decoration={brace},color=gray] (8.8,-1.3)--node[below]{$\wdth$}(-11,-1.3);
\draw[decorate,decoration={brace},color=gray] (-11-.22,-1.1+.22)--node[above left]{$\hte$}(-10/1.1-.2/1.1,1/1.1+.2/1.1);

\foreach\i in {-10,-9.8,...,8}{
\draw[color=gray]({\i*1.1},-1.1)--({\i/1.1},1/1.1);
}
\foreach\i in {-9.9,-9.7,...,7.9}{
\fill(\i,.5)circle(.1);
\draw(\i,.0)--(\i,.5);
}
\node[right,text width=2cm] at (9,.5){Degeneracy index};
\end{tikzpicture}

